Intruding with Words: Towards Understanding Graph Injection Attacks at the Text Level

Graph Neural Networks (GNNs) excel across various applications but remain vulnerable to adversarial attacks, particularly Graph Injection Attacks (GIAs), which inject malicious nodes into the original graph and pose realistic threats. Text-attributed graphs (TAGs), where nodes are associated with textual features, are crucial due to their prevalence in real-world applications and are commonly used to evaluate these vulnerabilities. However, existing research only focuses on embedding-level GIAs, which inject node embeddings rather than actual textual content, limiting their applicability and simplifying detection. In this paper, we pioneer the exploration of GIAs at the text level, presenting three novel attack designs that inject textual content into the graph. Through theoretical and empirical analysis, we demonstrate that text interpretability, a factor previously overlooked at the embedding level, plays a crucial role in attack strength. Among the designs we investigate, the Word-frequency-based Text-level GIA (WTGIA) is particularly notable for its balance between performance and interpretability. Despite the success of WTGIA, we discover that defenders can easily enhance their defenses with customized text embedding methods or large language model (LLM)--based predictors. These insights underscore the necessity for further research into the potential and practical significance of text-level GIAs.

==> Method.tex <==
\section{LLMGIA: A unified LLM-based GIA framework} \label{Sec:5 LLMGIA}
\begin{figure*}[htbp]
\centering
\includegraphics[width=0.88\textwidth]{figs/Framework_Neww.pdf}
\caption{Framework of LLMGIA. The color shade of a node reflects the confidence that the node is correctly classified. The darker the color, the higher the confidence. It is designed with four components: (1) \emph{Example node selection} to select suitable nodes with high-quality text. (2) \emph{Victim nodes \& class selection} to select nodes and classes that are easy to attack. (3) \emph{Raw text generation} generate interpretable and unnoticeable text for injected nodes. (4) \emph{Structure optimization} optimize the connections between the injected nodes and
the original graph.}
\label{fig:Framework}
\end{figure*}
In the previous section, we introduced GTA and TGA, two GIAs based on LLMs. 
By providing varied prompts, these methods generate harmful text for injected nodes, achieving effective attacks while ensuring the interpretability of features. 
In this section, we dive into unnoticeability further to better meet practical scenarios and propose an LLM-based GIA framework - LLMGIA.

\begin{algorithm}[htp!]
\SetAlgoLined
\SetNoFillComment
\DontPrintSemicolon
\SetAlgoNoLine % This removes the vertical line
\SetAlgoNoEnd % This removes the end keywords
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\SetKwInOut{Parameter}{Parameter}
\caption{LLMGIA: A Unified Large Language Model-based Graph Injection Attack Framework} \label{alg:LLMGIA}
\Input{Graph $\mathcal{G} = \left(\mathcal{V}, \mathcal{E}, \{s_i\}\right)$, Class set $C$, Number of injected nodes $N_{\text{inj}}$, Number of target nodes $|\mathcal{V}_T|$.}
\Output{Attacked Graph $\mathcal{G}' = (\mathcal{V}', \mathcal{E}', \{s_i\}')$}
\Parameter{Confidence threshold $\theta$, Average degree $d_{\text{avg}}$, Text length range $[l_{\text{min}}, l_{\text{max}}]$, Sequential step $st$, Number of sampled example nodes $n_e$, Number of sampled victim nodes $n_v$, Hyperparameter $\gamma$.}

\tcc{Initialization}
$\mathcal{V}' \gets \mathcal{V}$; $\mathcal{E}' \gets \mathcal{E}$; $\{s_i\}' \gets \{s_i\}$\;  
$\mathcal{V}_{\text{ex}} \gets \emptyset$; $\mathcal{V}_{\text{vict}} \gets \emptyset$; $\mathcal{V}_{\text{inj}} \gets \emptyset$; 
$\{s_i\}_{\text{inj}} \gets \emptyset$\;
$N_{\rm{Total}} \gets 0$; 
\tcp*[r]{Number of Already injected nodes}

\tcc{Example Nodes Selection}
\For{$v_i \in \mathcal{V}$}{
    \If{$\text{Confidence}(v_i) > \theta$ \textbf{and} $\text{Degree}(v_i) < d_{\text{avg}}$ \textbf{and} $\text{Length}(s_i) \in [l_{\text{min}}, l_{\text{max}}]$}{
        $\mathcal{V}_{\text{ex}} \gets \mathcal{V}_{\text{ex}} \cup \{v_i\}$\;
    }
}

\tcc{Sequential Generation}
\While{$N_{\text{Total}} < N_{\text{inj}}$}{
    $n \gets \min(N_{\text{inj}} - N_{\text{Total}}, \lfloor N_{\text{inj}}*{st} \rfloor)$\;
    $n_t \gets n \cdot \gamma$\;

    \tcc{Victim Nodes \& Class Selection}
    \For{$v \in \mathcal{V}$}{
        $\text{Score}(v) \gets \text{CalculateVulnerableScore}(v)$\;
    }
    \For{$c \in C$}{
        $\text{AvgScore}(c) \gets \text{AverageScore}(\text{top } n_t \text{ nodes in } c)$\;
    }
    $c_{\text{target}} \gets \text{class with highest } \text{AvgScore}$\;
    $\mathcal{V}_{\text{vict}} \gets \text{top } n_t \text{ nodes in } c_{\text{target}}$\;

    \tcc{Raw Text Generation}
    $\mathcal{V}_{\text{inj}}, \{s_i\}_{\text{inj}} \gets \text{GenerateText}(n, \mathcal{V}_{\text{ex}}, \mathcal{V}_{\text{vict}}, n_e, n_v)$\;

    \tcc{Structure Optimization}
    \eIf{Uniform Strategy}{
        $\mathcal{E}_{\text{inj}} \gets \text{FormUniformEdges}(\mathcal{V}_{\text{inj}}, \mathcal{V}_{\text{vict}})$\;
    }{
        $\mathcal{E}_{\text{inj}} \gets \text{FormWeightedEdges}(\mathcal{V}_{\text{inj}}, \mathcal{V}_{\text{vict}}, \text{Score})$\;
    }
    $\mathcal{V}' \gets \mathcal{V'} \cup \mathcal{V}_{\text{inj}}$;
    $\mathcal{E}' \gets \mathcal{E'} \cup \mathcal{E}_{\text{inj}}$\;
    $\{s_i\}' \gets \{s_i\}' \cup \{s_i\}_{\text{inj}}$

    $\mathcal{V}', \mathcal{E}' \gets \text{AdaptiveInjection}(\mathcal{V}', \mathcal{E}', \{s_i\}')$\;
    $N_{\text{Total}} \gets N_{\text{Total}} + n$\;
    \hrulefill % This adds a horizontal rule to indicate the end of the for loop block
}
\Return{Attacked Graph $\mathcal{G}' = (\mathcal{V}', \mathcal{E}', \{s_i\}')$}\;
\end{algorithm}
\subsection{Unnoticability of Prompt Strategies} \label{Sec:5.1 uno}
We divide the unnoticeability requirement for injected text into two parts: 
\textbf{1)} The text of injected nodes must exhibit diversity. 
Injecting a batch of nodes with similar features would also be easily noticed. 
Hence, it is vital to ensure a certain level of feature diversity among injected nodes.
\textbf{2)} The text of injected nodes must maintain high similarity with the text of nodes in the original graph. 
If injected nodes are significantly different from existing nodes, they would be easily detected by the defender.
To better quantize the unnoticeability of injected nodes, we first perform t-SNE dimensionality reduction~\cite{tsne_Van_08} on all node embeddings $\X'$ and denoted the output as $\X^t = \left[\X^t; \X_{\rm{inj}}^t\right]^\top$.
We then propose \textbf{Diversity Score (Div.)} and \textbf{Indistinguishability Score (Ind.)}  as metrics for unnoticeability based on t-SNE outputs $\X^t$. \\
\textbf{Diversity Score.} For each injected node pair $v_i$ and $v_j$ with embedding $\M_i = \X_{\rm{inj}}^t[i, :]$ and $\M_j = \X_{\rm{inj}}^t[j, :]$, we calculate their cosine similarity as $\cos(v_i, v_j) = \frac{\M_i \cdot \M_j}{\left\|\M_i\right\|\left\|\M_j\right\|}$.
Then, the Diversity Score is defined as:
\begin{align}
    \textbf{\textrm{Div.}} = \frac{1}{\binom{n}{2}} \sum_{i \neq j} \sum_{v_i, v_j \in \mathcal{V}_{\mathrm{inj}}} \cos(v_i, v_j).
\end{align} 
A lower diversity score means a lower similarity among the injected nodes, implying better diversity. \\
\textbf{Indistinguishability Score.} For each injected node $v_i$ with embedding $\M_i = \X_{\rm{inj}}^t[i, :]$, we find its nearest neighbor in the embedding matrix of original nodes $\X^t$. 
Then, we use the average distance of the injected nodes to their nearest neighbors as the Indistinguishability Score. 
Formally, for distance metric $d( , )$, the score is: 
\begin{align}
    \textbf{\textrm{Inv.}} = \frac{1}{N_{\rm{inj}}} \sum_{i=1}^{N_{\rm{inj}}} \min _{\boldsymbol{x} \in \X^t} d\left(\M_i, \boldsymbol{x}\right).
\end{align}
Here, we use Euclidean distance as the metric. 
A lower score means the injected nodes have a shorter distance to nodes in the original graph, indicating better indistinguishability. \\
We test the Diversity and Indistinguishability of GTA and TGA in Table~\ref{tab:properties}. 
Combined with the results in Table~\ref{tab:Vanilla GIA}, we see that there exists a clear trade-off between performance and unnoticeability. 
\begin{table}[htp!]
\vspace{-1em}
\centering
\caption{Diversity Score and Indistinguishability Score for LLM-based GIAs. Both metrics are better for lower values.}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lrrrrrr}
\toprule
\textbf{Attack}             & \multicolumn{2}{c}{\textbf{Cora}} & \multicolumn{2}{c}{\textbf{Citeseer}} & \multicolumn{2}{c}{\textbf{Pubmed}} \\
& Div.$(\downarrow)$ & Ind.$(\downarrow)$  & Div.$(\downarrow)$  & Ind.$(\downarrow)$ & Div.$(\downarrow)$  & Ind.$(\downarrow)$ \\
\midrule
GTA-Random               & 0.996     & 4.729                 & 0.996             & 8.394               & 0.979             & 4.059               \\
GTA-Mixing               & 0.997     & 4.037                 & 0.990             & 4.926               & 0.669             & 1.419               \\
GTA-Sample               & 0.328     & 2.101                 & 0.649             & 4.008               & 0.028             & 0.944               \\
TGA-Random               & 0.959     & 4.675                 & 0.969             & 14.724              & 0.988             & 6.282               \\
TGA-Mixing               & 0.994     & 3.411                 & 0.994             & 3.686               & 0.557             & 1.309               \\
TGA-Sample               & \textbf{0.056}     & \textbf{0.959}                 & \textbf{0.024}             & \textbf{1.631}               & \textbf{0.006}             & \textbf{0.553}               \\
\midrule
LLMGIA-Uniform           & 0.639     & 2.512                 & 0.519             & 4.580               & 0.594             & 1.836               \\
LLMGIA-Weighted          & 0.560     & 3.140                 & 0.453             & 3.790               & 0.388             & 1.765               \\
\bottomrule
\end{tabular}
}
\label{tab:properties}
\end{table}
Random Prompt and Mixing Prompt Generally hold better performance than Sample Prompt across datasets, but Mixing Prompt fails to generate diverse content, and Random Prompt fails to generate either diverse or similar content to the nodes in the original graph. 
A better LLM-based GIA should stand in the middle, introducing representative content from the original dataset as a hint while generating confusing content at the same time.

\subsection{Our Method: LLMGIA}
Based on the insights gained from prior experiments of GTA and TGA, as well as considerations regarding prompt unnoticeability, we propose LLMGIA, a unified LLM-based GIA framework as shown in Figure~\ref{fig:Framework}.
The pseudo-code of LLMGIA is presented in Algorithm~\ref{alg:LLMGIA}. 
The framework aims to ensure desirable attack performance while maintaining a high degree of unnoticeability. 
LLMGIA comprises four main components: Example Nodes Selection, Victim Nodes \& Class Selection, Raw Text Generation, and Structure Optimization. \\
\textbf{Example Nodes Selection.} To ensure unnoticeability, it is essential to include high-quality text in the prompts provided to LLM from nodes in the original graph. 
In LLMGIA, we identify suitable example nodes based on the following criteria: 
1) The text of the node should be correctly classified with high confidence, indicating high-quality text reflective of its class characteristics. 
In the implementation, we will adopt a surrogate GNN (we use a three-layer GCN) to provide a confidence score for each node in the graph and select labeled nodes that are rightly classified with high confidence.
2) The node should have a relatively low degree. 
Nodes with high degrees might derive their classification confidence more from high-quality neighboring nodes rather than their own text. 
In practice, we filter out nodes with degrees higher than the average. 
3) The text length of the node should be appropriate. 
Overly long prompts would be challenging for LLM to understand, and too short text might lack representativeness of the corresponding class.
So, we only keep nodes with the text of medium length in the example node-set. \\
\textbf{Victim Nodes \& Class Selection.} 
In LLM-based GIA, it is impractical to update the features of injected nodes frequently, considering the high cost and time to query an LLM.
Therefore, we have devised an iterative strategy for selecting victim nodes and generating corresponding prompts. 
Drawing from~\cite{HAO_Chen_22}, we calculate a vulnerable score based on ATDGIA for each node in the target node set in each round. 
Specifically, lower classification confidence by the surrogate GNN and a smaller node degree contribute to a higher vulnerable score. 
Denote the number of iterations as $T$ and the number of nodes to be injected in each round as $n$.
In the current iteration, we choose the target class based on the class with the highest average scores among the top $n_t = n*\gamma$ most vulnerable nodes, where $\gamma \ge 1$ is a hyperparameter.
The $n_t$ nodes with the highest vulnerable score within the target class are chosen as victim nodes. 
Categorizing by the class during generation is advantageous as it ensures effective attacks on nodes of the current class while maintaining diversity across different iterative rounds. \\
\textbf{Raw Text Generation.}
In this part, we randomly select nodes within and outside the target class from the example node-set.
We extract the text of these nodes as positive and negative samples to help LLM understand the characteristics of the target class.
We then sample the nodes from the victim nodes, using their text to help LLM understand the nodes it is going to confuse.
In the prompt, we use the integrated prompt to instruct the LLM to generate text similar to the example node yet not belonging to the target class and potentially classifiable into any of the remaining categories. 
Detailed prompts are left in the Appendix~\ref{App:Prompt Design}. \\
\textbf{Structure Optimization.} Drawing from experiences in GTA and TGA, structural optimization is a crucial step in enhancing performance. 
We first initialize edges based on the vulnerable scores, using either uniform or weighted strategies. 
In the uniform strategy, injected nodes randomly form edges with selected victim nodes with equal probability. 
In the weighted strategy, injected nodes form edges with victim nodes with a probability distribution based on vulnerable scores, indicating a higher likelihood of connecting with nodes having higher vulnerable scores. 
Following initialization, we apply an adaptive injection method for fine-tuning the structure. 
In practice, we employ a meta-gradient-based adaptive injection method~\cite{Metattack_Zugner_19}.

\subsection{Experiments}
\textbf{Performance.}
For our proposed LLMGIA, we provide two variants LLMGIA-Uniform and LLMGIA-Weighted, corresponding to the two structure initialization strategies.
The preparation of datasets and evaluation protocol follows the same setup as in Section~\ref{Sec:4.2Exp}.
We set the sequential step $st$ being chosen from $\{0.01, 0.05\}$, and $\gamma$ being chosen from $[1.0, 1.5, 2.0]$. 
The results are summarized in Table~\ref{tab:LLMGIA}. 
Full results, including LLM-based GIAs against more defense models, are left in Appendix~\ref{App:Full results}. 
\begin{table}[htp!]
\centering
\caption{Comparison of LLM-based GIA Performance across Cora, CiteSeer, and PubMed Datasets.}
\label{tab:LLMGIA}
\begin{tabular}{lccc}
\toprule
Model & Cora & CiteSeer & PubMed \\
\midrule
Clean & 89.12 $\pm$ 0.44 & 76.60 $\pm$ 0.52 & 88.65 $\pm$ 0.18 \\
\midrule
GTA-Random & 86.35 $\pm$ 0.59 & 75.45 $\pm$ 0.56 & 77.39 $\pm$ 2.05\\ 
GTA-Mixing & 86.31 $\pm$ 0.33 & 75.15 $\pm$ 0.41 & 81.28 $\pm$ 0.89\\ 
GTA-Sample & 86.00 $\pm$ 0.47 & 74.96 $\pm$ 0.43 & 77.32 $\pm$ 0.97\\ 
TGA-Random & 83.58 $\pm$ 1.22 & 73.42 $\pm$ 0.78 & \textbf{72.03 $\pm$ 2.36}\\
TGA-Mixing & 84.12 $\pm$ 1.34 & 74.06 $\pm$ 0.40 & 79.47 $\pm$ 0.46\\
TGA-Sample & 86.19 $\pm$ 0.55 & 74.69 $\pm$ 0.44 & 78.09 $\pm$ 0.51\\
\midrule
LLMGIA-Uniform & \textbf{82.62 $\pm$ 0.80} & \underline{72.04 $\pm$ 0.55} & 74.78 $\pm$ 0.48\\ 
LLMGIA-Weighted & \underline{83.48 $\pm$ 0.53} & \textbf{71.42 $\pm$ 0.59} & \underline{74.33 $\pm$ 0.50}\\
\bottomrule
\end{tabular}
\end{table}

From the results, we see that the LLMGIA framework generally outperforms naive LLM-based GIAs except on the dataset PubMed. 
Uniform and Weighted strategies both work well but differ a little
depending on the nature of the datasets. \\
\textbf{Unnoticability.}
We test the unnoticeability of LLMGIA following the same setting in Section~\ref{Sec:5.1 uno}.
The results are summarized in Table~\ref{tab:properties}.
We can see that LLMGIA shows better diversity and indistinguishability than the ones using Random Prompt and Mixing Prompt but is slightly inferior to the ones using Sample Prompt.
In Figure~\ref{fig:Property}, we visualize the relationship between unnoticability and performance.
Based on the definition of unnoticeability metrics, nodes in the lower left region hold better unnoticeability.
We set the node size as $\textrm{Performance} = \textrm{exp}\left(1 - acc/100 \right) * 170$, where $acc$ is the classification accuracy in Table~\ref{tab:LLMGIA}.
So a larger node size in the figure indicates a better performance.
From the figure, a clear trade-off among the prompts can be seen. 
Nodes of LLMGIA lie in the center of the figure with larger node sizes compared to most baselines, demonstrating desirable performance while enjoying the best attack performance.
\begin{figure}[htp!]
\centering
% \begin{subfigure}[b]{0.156\textwidth}
%    \centering
%    \includegraphics[width=\textwidth]{figs/Property_Cora.pdf}
%    \caption{Cora}
%    \label{fig:Prop_cora}
% \end{subfigure}
% \begin{subfigure}[b]{0.156\textwidth}
%    \centering
%    \includegraphics[width=\textwidth]{figs/Property_CiteSeer.pdf}
%    \caption{CiteSeer}
%    \label{fig:Prop_citeseer}
% \end{subfigure}
% \begin{subfigure}[b]{0.156\textwidth}
%    \centering
%    \includegraphics[width=\textwidth]{figs/Property_PubMed.pdf}
%    \caption{PubMed}
%    \label{fig:Prop_pubmed}
% \end{subfigure}

\includegraphics[width=0.48\textwidth]{figs/Property.pdf}
\caption{Performance versus Unnoticability on Cora and CiteSeer. 
Larger node size indicates better performance.
LLMGIA well balances the attack performance and unnoticability. See Appendix~\ref{App:Visual Pubmed} for the PubMed dataset.}
\label{fig:Property}
\end{figure}

We also include an ablation study of LLMGIA with respect to its hyperparameters in Appendix~\ref{App:Hyperparams for LLMGIA}.
The result demonstrates that LLMGIA is insensitive to the choice of hyperparameters.

